Towards General Visual-Linguistic Face Forgery Detection

Deepfakes are realistic face manipulations that can pose serious threats to security, privacy, and trust. Existing methods mostly treat this task as binary classification, which uses digital labels or mask signals to train the detection model. We argue that such supervisions lack semantic information and interpretability. To address this issues, in this paper, we propose a novel paradigm named Visual-Linguistic Face Forgery Detection(VLFFD), which uses fine-grained sentence-level prompts as the annotation. Since text annotations are not available in current deepfakes datasets, VLFFD first generates the mixed forgery image with corresponding fine-grained prompts via Prompt Forgery Image Generator (PFIG). Then, the fine-grained mixed data and coarse-grained original data and is jointly trained with the Coarse-and-Fine Co-training framework (C2F), enabling the model to gain more generalization and interpretability. The experiments show the proposed method improves the existing detection models on several challenging benchmarks. Furthermore, we have integrated our method with multimodal large models, achieving noteworthy results that demonstrate the potential of our approach. This integration not only enhances the performance of our VLFFD paradigm but also underscores the versatility and adaptability of our method when combined with advanced multimodal technologies, highlighting its potential in tackling the evolving challenges of deepfake detection.

==> table/ablation4.tex <==
\begin{table}[!t]
    \centering
    \renewcommand\arraystretch{1.1}
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{c|cc|cc}
        \hline
        %\multicolumn{4}{|c|}{GCD-AVG}\\
        %\hline
        \multirow{2}*{Method} & \multicolumn{2}{c|}{Celeb-DF}&
        \multicolumn{2}{c}{DFDC-P}  \\
        \cline{2-5}
        % \cmidrule{2-5}
        & AUC& EER &AUC& EER \\
        \hline
        % Prompt1&77.21&29.55&77.39&30.36\\
        Prompt 1&82.17&25.18&79.19&26.13\\
        Prompt 2&81.60&26.78&82.04&26.26\\
        Prompt 3&83.32&24.40&83.09&24.90\\
        Prompt 4&\textbf{84.80}&\textbf{22.73}&\textbf{84.74}&\textbf{23.43}\\
        \hline
    \end{tabular}
    }
    \vspace{-2pt}
    \caption{Ablation of different coarse-grained prompts.}
    \label{table:ab4}
\end{table}


==> table/alg_test.tex <==

\begin{algorithm}[!h]
    
    \caption{Testing period}
    \begin{algorithmic}[1]%显示行号
        \Require{Coarse-grained label set C, Fine-grained prompt set P, image encoder $E_i$, text encoder $E_t$, input image $x$.}
        \State  $l_C=E_t(C)$ 
        \State  $l_F=E_t(P)$ 
        \State  $v_x=E_i(x)$
        \State $coarse\_result,\_ = argmax(s(v_x,l_C)$
        \State Use $coarse\_result$ calculate AUC and EER
        \If {Need fine-grained result}
            \State $fine\_result,index = argmax(s(v_x,l_F)$
            \State \textbf{Return} coarse\_result, AUC, EER, P[index]
        \Else
            \State \textbf{Return} coarse\_result, AUC, EER
        \EndIf
    \end{algorithmic}
    \label{alg:test}
    
\end{algorithm}

==> table/tab2_c40.tex <==

% \begin{table}[t!]
    
%     \renewcommand\arraystretch{1.4}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{ccc}
%         \hline
%         Method&FF++&Celeb-DF\\
%         \hline
%         Two-stream \cite{zhou2017two}&70.10&53.80\\
%         Meso-4\cite{afchar2018mesonet}&84.70&54.80\\
%         Mesoinception4\cite{afchar2018mesonet}&83.00&53.60\\
%         FWA\cite{li2018exposing}&80.10&56.90\\
%         DSP-FWA\cite{li2018exposing}&93.00&	64.60\\
%         Xception\cite{rossler2019faceforensics++}&95.50&65.50\\
%         Multi-task\cite{nguyen2019multi}&76.30&54.30\\
%         % Capeule\cite{nguyen2019use}&96.60&57.50\\
%         SMIL\cite{li2020sharp}&96.80&56.30\\
%         Two Branch\cite{masi2020two}&93.18&	73.41\\
%         EN-b4\cite{dolhansky2020deepfake}&96.39	&71.10\\
%         MAT\cite{zhao2021multi}&96.41&72.50	\\
%         GFF\cite{luo2021generalizing}&95.73&74.12\\
%         SPSL\cite{liu2021spatial}&96.91&	76.88\\
%         \hline
%         Ours&\textbf{96.97}&\textbf{81.00}\\
%         \hline
%     \end{tabular}
%     }
%      \vspace{-2pt}
%     \caption{Cross-dataset evaluation from FF++(LQ) to deepfake class of FF++ and Celeb-DF in terms of AUC. Some results
%     are from~\cite{masi2020two}, and the bold results are the best.}
%     \label{table:2}
% \end{table}

% \begin{table}[t!]
    
%     \renewcommand\arraystretch{1.2}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|c}
%         \hline
%         Method&Celeb-DF(AUC)\\
%         \hline
%         Two-stream \cite{zhou2017two}&53.80\\
%         Meso-4\cite{afchar2018mesonet}&54.80\\
%         Mesoinception4\cite{afchar2018mesonet}&53.60\\
%         FWA\cite{li2018exposing}&56.90\\
%         Xception\cite{rossler2019faceforensics++}&65.50\\
%         Multi-task\cite{nguyen2019multi}&54.30\\
%         % Capeule\cite{nguyen2019use}&57.50\\
%         DSP-FWA\cite{li2018exposing}&	64.60\\
%         SMIL\cite{li2020sharp}&56.30\\
%         Two Branch\cite{masi2020two}&	73.41\\
%         EN-b4\cite{dolhansky2020deepfake}&71.10\\
%         MAT\cite{zhao2021multi}&72.50	\\
%         F3-Net\cite{qian2020thinking}&65.17 \\
%         SPSL\cite{liu2021spatial}&	76.88\\
%         \hline
%         Ours&\textbf{81.00}\\
%         \hline
%     \end{tabular}
%     }
%      \vspace{-2pt}
%     \caption{Low quality image }
%     \label{table:2}
% \end{table}

\begin{table}[t!]
    
    \renewcommand\arraystretch{1.1}
    \centering.
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{c|cc}
        \hline
        Method&\quad   FF++ \quad  \quad&Celeb-DF\quad\\
        \hline
        % Two-stream &70.10&53.80\\
        Meso-4&84.70&54.80\\
        Mesoinception4&83.00&53.60\\
        FWA&80.10&56.90\\
        % DSP-FWA&93.00&	64.60\\
        Xception&95.50&65.50\\
        Multi-task&76.30&54.30\\
        % Capeule\cite{nguyen2019use}&96.60&57.50\\
        SMIL&96.80&56.30\\
        Two Branch&93.18&	73.41\\
        EN-b4&96.39	&71.10\\
        Multi-Attention&96.41&72.50	\\
        GFF&95.73&74.12\\
        SPSL&96.91&	76.88\\
        \hline
        Ours&\textbf{96.97}&\textbf{81.00}\\
        \hline
    \end{tabular}
    }
     
    \caption{Cross-dataset evaluation from FF++(LQ) to deepfake class of FF++ and Celeb-DF in terms of AUC.}
    
    \label{table:2}
\end{table}

